ImageNet-Patch: A Dataset for Benchmarking Machine Learning Robustness against Adversarial Patches

Adversarial patches are optimized contiguous pixel blocks in an input image that cause a machine-learning model to misclassify it. However, their optimization is computationally demanding, and requires careful hyperparameter tuning, potentially leading to suboptimal robustness evaluations. To overcome these issues, we propose ImageNet-Patch, a dataset to benchmark machine-learning models against adversarial patches. It consists of a set of patches, optimized to generalize across different models, and readily applicable to ImageNet data after preprocessing them with affine transformations. This process enables an approximate yet faster robustness evaluation, leveraging the transferability of adversarial perturbations. We showcase the usefulness of this dataset by testing the effectiveness of the computed patches against 127 models. We conclude by discussing how our dataset could be used as a benchmark for robustness, and how our methodology can be generalized to other domains. We open source our dataset and evaluation code at https://github.com/pralab/ImageNet-Patch.

==> icub_old.tex <==
% %\documentclass[review]{elsarticle}
% %\documentclass[sort&compress,twocolumn,5p]{elsarticle}
% \documentclass[preprint,12pt]{elsarticle}

% \usepackage{setspace}
% \doublespacing

% % template for neurocomputing
% % chiedono di includere il doi nelle ref quando possibile

% \usepackage[utf8]{inputenc} %unicode support

% %\usepackage{lineno,hyperref}
% %\modulolinenumbers[5]

% \usepackage[table]{xcolor}
% \usepackage{subcaption}
% \usepackage{balance}
% \usepackage{amsmath,amssymb}
% \usepackage{url}
% \journal{Pattern Recognition}

% \bibliographystyle{elsarticle-num}

% \usepackage{color}
% \usepackage{xcolor}

% \usepackage{xspace}
% \usepackage{graphicx}
% \usepackage{longtable}
% \usepackage{caption}
% \usepackage{amsmath,amsthm}
% \usepackage{multirow}
% \usepackage{multicol}
% \usepackage{booktabs}
% \usepackage{url}
% \usepackage{pifont}
% \usepackage{color}
% \usepackage{supertabular}
% \usepackage[export]{adjustbox}

% \usepackage{algorithm}
% \usepackage{algorithmicx}
% \usepackage{algpseudocode}

% \usepackage{amsmath}
% \usepackage{amsthm,amsmath,amssymb}
% \usepackage{mathrsfs}
% \usepackage{bm}
% \usepackage{subcaption}
% \usepackage{hyperref}
% \usepackage{CJKutf8}

% \usepackage{cleveref}

% \floatname{algorithm}{Algorithm}
% \renewcommand{\algorithmicrequire}{\textbf{Input:}}
% \renewcommand{\algorithmicensure}{\textbf{Output:}}

% % for figure placement
% \renewcommand{\topfraction}{0.99}	% max fraction of floats at top
% \renewcommand{\bottomfraction}{0.99}	% max fraction of floats at bottom
% %   Parameters for TEXT pages (not float pages):
% \setcounter{topnumber}{9}
% \setcounter{bottomnumber}{9}
% \setcounter{totalnumber}{9}     % 2 may work better
% \setcounter{dbltopnumber}{9}    % for 2-column pages
% \renewcommand{\dbltopfraction}{0.99}	% fit big float above 2-col. text
% \renewcommand{\textfraction}{0.001}	% allow minimal text w. figs
% %   Parameters for FLOAT pages (not text pages):
% \renewcommand{\floatpagefraction}{0.001}	% require fuller float pages
% % N.B.: floatpagefraction MUST be less than topfraction !!
% \renewcommand{\dblfloatpagefraction}{0.001}	% require fuller float pages


% %our macro:
% \newcommand{\diff}[2]{\frac{\partial #1}{\partial #2}}
% %\newcommand{\vct}[1]{\ensuremath{\mathbf{#1}}}
% \newcommand{\vct}[1]{\ensuremath{\boldsymbol{#1}}}
% \newcommand{\mat}[1]{\ensuremath{\mathbf{#1}}}
% \newcommand{\set}[1]{\ensuremath{\mathcal{#1}}}
% \newcommand{\con}[1]{\ensuremath{\mathsf{#1}}}
% \newcommand{\tsum}{\ensuremath{\textstyle \sum}}
% \newcommand{\T}{\ensuremath{\top}}
% \newcommand{\mycomment}[1]{\textcolor{red}{#1}}
% \newcommand{\ind}[1]{\ensuremath{\mathbbm 1_{#1}}}
% \newcommand{\argmax}{\operatornamewithlimits{\arg\,\max}}
% \newcommand{\erf}{\text{erf}}
% \newcommand{\sign}{\text{sign}}
% \newcommand{\argmin}{\operatornamewithlimits{\arg\,\min}}
% \newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}


% \newcommand{\myparagraph}[1]{\smallskip \noindent \textbf{#1}}
% \newcommand{\ie}{{i.e.}\xspace}
% \newcommand{\eg}{{e.g.}\xspace}
% \newcommand{\etal}{{et al.}\xspace}
% \newcommand{\etc}{{etc.}\xspace}
% \newcommand{\aka}{{a.k.a.}\xspace}


% \begin{document}

% \begin{frontmatter}

% %\title{Detecting Adversarial Patches against the ICub Humanoid}
% %\title{Detecting Adversarial Patches in Open World Scenarios: A Case Study on the ICub Humanoid}
% \title{Adversarial Patches: A Dataset for Benchmarking the iCub Humanoid against Physical Attacks}



% \author[unica, pluribus]{Angelo Sotgiu}

% \author[unica]{Daniele Angioni}

% \author[unica]{Ambra Demontis\corref{mycorrespondingauthor}}
% \cortext[mycorrespondingauthor]{Corresponding author}
% \ead{ambra.demontis@unica.it}

% \author[unica]{Luca Demetrio}

% \author[unica]{Maura Pintor}

% \author[unica,pluribus]{Battista Biggio}

% \author[unige,pluribus]{Fabio Roli}

% \address[unica]{University of Cagliari, Italy}
% \address[unige]{University of Genoa, Italy}
% \address[pluribus]{Pluribus One, Italy}

% \begin{keyword}
% adversarial machine learning \sep adversarial patches \sep neural networks \sep defense \sep detection 
% \end{keyword}

% % max 150 words
% \begin{abstract}

% \end{abstract}

% \end{frontmatter}

% \section{Introduction}\label{sec1}

% Goal: Fornire un dataset di benchmark per valutare la robustezza dei sistemi di riconoscimento di immagini contro adversarial batches. Perchè il dataset sia utile a questo scopo, le adversarial patches devono avere i seguenti requisiti:
% \begin{itemize}
%     \item Deve portare alla classificazione dell'oggetto come appartenente alla classe scelta dall'attaccante
%     \item Non dono essere specifiche contro una determinata architettura ma devono generalizzare a diverse architetture
%     \item Devono poter essere robuste a diverse trasformazioni (scala, rotazione, traslazione) in modo che siano utilizzabili nel mondo reale.
%     \item Devono essere robuste rispetto al background
%     \item Deve generalizzare a diversi oggetti dello stesso tipo (non deve essere specifica per una determinata tazza ma deve funzionare per ogni tazza)
%     \item Deve essere facilmente stampabile (deve funzionare una volta stampata e mostrata ad una telecamera)
    
% \end{itemize}

% Contributions:
% \begin{itemize}
%     \item Un protocollo che può essere utilizzato per creare dataset di adversarial patch con i requisiti spiegati sopra.
%     \item Un dataset che può essere utilizzato come benchmark per valutare la robustezza dei sistemi di object recognition contro adversarial patches.
%     \item Un'analisi sperimentale che mostra la differenza di efficacia delle adversarial patches a seconda dei modelli contro la quale sono calcolatee
%     \item Un'analisi sperimentale che valuta l'efficacia delle difese al SoA nel rilevare questi attacchi 
%     \item Un'analisi dell'efficacia delle adversarial patches generate nel real world
% \end{itemize}


% \section{The iCub Humanoid} 
% \label{sec:iCub}

% \mycomment{questo testo l'ho masso come placeholder, lo devo rivedere}
% Our case study focuses on the computer vision system of the iCub humanoid~\cite{metta2008icub,pasquale2015teaching}. We consider a cognitive humanoid robotic platform because the security of those systems is particularly relevant as they have often physical interactions with humans. The damage caused by their insecurity is therefore especially concerning. The visual recognition system of iCub enables the robot to detect and recognize people and objects. The robot is trained by a human teacher that provides it with examples and verbal annotations. After the training, the robot is asked to classify the object and faces that its sees. If the robot is wrong i.e., if its prediction is uncorrect because the either, the object belongs to a never-seen-class or because the model learned by the robot is not accurate, the teacher can interact with the robot providing it the correct label of the misclassified object. The robot can therefore update its classification model through online or incremental learning techniques (\eg, eventually also expanding the set of known object classes). In this way the robot can learn from its experience improving its capabilities. 

% The computer vision of iCub, is shown in Fig.~\ref{fig:iCub}, relies on deep learning technologies. Given the limited hardware and power resources of the robot, it wouldn't have been possible to train a deep neural network using the robot hardware. iCub exploits therefore a deep neural network~\cite{alex12-nips} pre-trained on the ImageNet dataset~\cite{russakovsky15} for extracting a set of deep features. Those features are extracted by the highest convolutional layers of the network and are used by the robot to represent each input image. 

% As described in Fig.~\ref{fig:iCub}, this deep feature vector is then classified using a separate classifier, which can be retrained online in an efficient manner when feedback from the human annotator is received.b
% In particular, in~\cite{pasquale2015teaching} this classifier is implemented using a one-versus-all scheme to combine a set of $\con c$ linear classifiers, being $\con c$ the number of known classes.
% Let us denote the pixel values of the input image (in raster-scan order) with $\vct x \in \set X \subseteq \mathbb R^{\con d}$ (where $\con d = 128 \times 128 \times 3$), and the discriminant functions of the aforementioned one-versus-all linear classifiers as $f_{1}(\vct x), \ldots, f_{\con c}(\vct x)$. Accordingly, the predicted class $c^{\star}$ is determined as the class whose discriminant function for that sample is maximum:
% \begin{align}
% c^{\star} = \argmax_{k=1, \ldots, \con c}  f_k(\vct x ) \, .
% \label{eq:ev2}
% \end{align}
% The linear classifiers used for this purpose include Support Vector Machines (SVMs) and Recursive Least Square (RLS) classifiers, as both can be efficiently updated online~\cite{pasquale2015teaching}.
% Notably, previous work has shown that replacing the softmax layer in deep networks with a multiclass SVM can be effective also in different applications~\cite{tang13-deepsvm}.


% \section{The Adversarial iCub Patches Dataset}

% \subsection{Crafting Adversarial Patches}
% Qui dobbiamo spiegare come creare le adversarial patches con i requisiti spiegati sopra (mostrare la funzione obiettivo che utilizzeremo e descriverla)

% Questa deve essere:
% \begin{itemize}
% \item targeted 
% \item il loss che è una media del loss su diversi modelli (per avere invarianza in base al modello)
% \item il loss dovrebbe essere invariante rispetto a varie trasformazioni applicate all'immagine.
% \item avere dei regolarizzatori per ottenere stampabilità? Servono?
% \item per ogni calasse deve essere mediata su immagini di diversi oggetti e con diverso background
% \end{itemize}

% \subsection{The Protocol to Create an Adversarial Patches Dataset}
% Qui dobbiamo spiegare come va creato il dataset. Quali sono i requisiti del dataset dal quale partire e come procedere?
% Il dataset deve necessariamente contenere immagini di diversi oggetti e con diverso background. \\
% \\
% Si calcolano le patch con funzioone obiettivo vista sopra. \\
% Si testa l'efficacia delle patch in digitale (dobbiamo spiegare come) \\
% Si riacquisiscono \\ 
% Si testa l'efficacia delle patch nel real world \\ 

% \subsection{The Created Datasets}
% Qui dovremmo illustrare le caratteristiche dei dataset creati. 
% Quante immagini, quali size delle patch abbiamo considerato, etc. 
% Qui potremmo descrivere i dataset creati (quante immagini, quali size delle patch, mettere alcune immagini etc.)\\

% Come dataset di base possiamo usare iCubWorld Transformations cropped. 
% Contiene 20 categorie e 10 oggetti per ogni categoria. Le immagini sono inoltre acquisite con diverse trasformazioni:
% \begin{itemize}
% \item 2D ROTATION: rotazione parallela alla camera
% \item 3D ROTATION: out-of-plane rotations
% \item SCALING changing the object's scale with respect to the cameras.
% \item BACKGROUND CHANGE
% \end{itemize}
% Possiamo usare 5 oggetti per creare il dataset e 5 per valutare. 
% Per quanto riguarda i modelli possiamo creare due dataset calcolando gli attacchi su:
% \begin{itemize}
%     \item 3 modelli non robusti
%     \item 3 modelli robusti
% \end{itemize}
% Poi andremo a far vedere che le patches create su quelli robusti sono più efficaci e quindi andremo a rilasciare solo quello. 

% Per quanto riguarda le trasformazioni potremmo addestrare gli oggetti su quelle singole e poi testare sul MIX che contiene immagini alle quali sono state applicate combinazioni di trasformazioni. 

% \section{Experimental Analysis}\label{sec1}
% Qui andremmo a presentare l'analisi sperimentale

% \subsubsection{Experimental Protocol}
% Qui dobbiamo dire quali modelli usiamo per il test, quali detectors etc. 

% \myparagraph{Detectors.} Qui dovremmo considerare solo detector che non fanno adversarial training:
% \begin{itemize}
%     \item PatchCleanser 
%     \item DNR
%     \item una difesa certificata. Quale? 
% \end{itemize}

% \subsubsection{Experimental Results}

% \subsection{Experiments in the Digital World}

% \myparagraph{Genearalization to other Models and Objects}
% Qui dobbiamo verificare se le patches create generalizzando ad altri modelli e ad altri oggetti. Potremmo avere:
% \begin{itemize}
% \item una tabella una che mostra l'accuracy su 6 modelli (3 considerati durante l'addestramento e 3 no). Modello usato per calcolo patch vs modello test. 
% \item qualcosa che mostra l'accuracy sui vari oggetti (su quelli usati per calcolo patch e su quelli non usati). (magari un istogramma e poi mostriamo la media dei due gruppi) 
% \end{itemize}

% \myparagraph{Effectiveness against Detectors}
% Qui potremmo testare l'efficacia dei due dataset generati (quello generato su modelli non robusti e quello generato su modelli robusti) contro detectors al soa. 

% Per questi esperimenti possiamo testare direttamente su oggetti e modelli che non conosce. 

% \subsection{Experiments in the Real World}

% Qui potremmo ripetere quanto sopra con il dataset di adversarial patches in real world (quelle stampate e riacquisite)

% \myparagraph{Genearalization to other Models and Objects}

% \myparagraph{Effectiveness against Detectors}

% \section{Related Work }\label{sec1}
% Qui potremmo parlare del dataset APRICOT 

% \section{Conclusions and Future Work}\label{sec1}


% %%=============================================================%%
% %% Sample for another appendix section			       %%
% %%=============================================================%%

% %% \section{Example of another appendix section}\label{secA2}%
% %% Appendices may be used for helpful, supporting or essential material that would otherwise 
% %% clutter, break up or be distracting to the text. Appendices can consist of sections, figures, 
% %% tables and equations etc.


% \bibliography{addref,bibDB}% common bib file

% \end{document}
% \ead{ambra.demontis@unica.it} 


